Mirrored Light Field Video Camera Adapter

This paper proposes the design of a custom mirror-based light field camera adapter that is cheap, simple in construction, and accessible. Mirrors of different shape and orientation reflect the scene into an upwards-facing camera to create an array of virtual cameras with overlapping field of view at specified depths, and deliver video frame rate light fields. We describe the design, construction, decoding and calibration processes of our mirror-based light field camera adapter in preparation for an open-source release to benefit the robotic vision community.

==> ctable/README <==
|
-------:|:--------------------------------------
 ctable:| Flexible typesetting of table and figure floats using key/value directives
Version:| 1.31
 Author:| Wybo Dekker
 E-mail:| wybo@dekkerdocumenten.nl
License:| Released under the LaTeX Project Public License v1.3c or later
    See:| http://www.latex-project.org/lppl.txt

Short description:
ctable.sty provides commands to easily typeset centered or left or right
aligned tables and (multiple-)figure floats, with footnotes. Instead of an
environment, a command with 4 arguments is used; the first is optional and
is used for key,value pairs generating variations on the defaults and
offering a route for future extensions.

Full documentation:
https://bitbucket.org/wybodekker/ctable/downloads/ctable.pdf

Installation:
Execute the inst script with the --help option for more information.

Changes in version 1.31:
 - comments about tmark in captions
 - use expandonce from etoolbox
 - use \AtBeginDocument, not \AtEndPreamble from etoolbox
   (problems with tikz)


==> ctable/doc/01a <==
\ctable[caption = a table]{c}{
}{\FL Table's first row\LL}


==> ctable/doc/01b <==
\newcommand{\F}[1]{
  \includegraphics[width=\hsize]{#1}
}
\newcolumntype{H}[1]{>{\hsize=#1\hsize}X}
\ctable[
  caption = a figure,
  figure, botcap,
  width=.4\hsize,
]{H{.4}H{.6}}{}{\FL
  \F{penguin}& \F{lion}\LL
}


==> ctable/doc/02k <==
\ctable[
  caption = Centered,
]{c}{}{\FL Table's first row\LL}


==> ctable/doc/02l <==
\ctable[
  caption = Left,
     left
]{c}{}{\FL Table's first row\LL}


==> ctable/doc/02m <==
\ctable[
  caption = Right,
    right
]{c}{}{\FL Table's first row\LL}


==> ctable/doc/03a <==
\ctable[
  caption = Caption,
]{c}{}{\FL Table's first row\LL}


==> ctable/doc/03b <==
\ctable[
    caption =  Caption,
captionskip = 1ex,
]{c}{}{\FL Table's first row\LL}


==> ctable/doc/04a <==
\ctable[
  caption = Caption,
   botcap
]{c}{}{\FL Table's first row\LL}


==> ctable/doc/04b <==
\ctable[
    caption =  Caption,
captionskip = -2ex,
     botcap
]{c}{}{\FL Table's first row\LL}


==> ctable/doc/05a <==
\ctable[
  caption = a lengthy caption
]{c}{}{\FL row1\LL}


==> ctable/doc/05b <==
\ctable[
  mincapwidth = 40mm,
  caption = a lengthy caption
]{c}{\tnote{this is a footnote}}
{\FL row1\tmark\LL}


==> ctable/doc/05c <==
\ctable[
  mincapwidth = 40mm,
  footerwidth,
  caption = a lengthy caption
]{c}{\tnote{footnote}}
{\FL row1\tmark\LL}


==> ctable/doc/06a <==
\ctable[framerule=.1pt, maxwidth=3cm
]{lX}{}{\FL 1 & first row\LL}



==> ctable/doc/06b <==
\ctable[framerule=.1pt, maxwidth=3cm
]{lX}{}{\FL 1 & test\LL}



==> ctable/doc/07a <==
\ctable{c}{
  \tnote{First footnote}
  \tnote[b]{Second footnote}
}{\FL Table's\tmark\ first\tmark[b]\ row\LL}



==> ctable/doc/07b <==
\ctable[nosuper]{c}{
  \tnote[a.]{First footnote}
  \tnote[b.]{Second footnote}
}{\FL Table's\tmark\ first\tmark[b]\ row\LL}



==> ctable/doc/08a <==
\ctable[
  caption = Frame,
]{c}{}{\FL Table's first row\LL}


==> ctable/doc/08b <==
\ctable[
  caption = Frame,
  framerule = 2pt,
  framefg = .8 0 0
]{c}{}{\FL Table's first row\LL}


==> ctable/doc/09b <==
\ctable[
  caption = Frame,
  framerule = 1pt,
  framefg = .8 0 0,
  framesep=10pt
]{c}{}{\FL Table's first row\LL}



==> ctable/doc/10a <==
\ctable[
  caption = Frame,
  framebg = 1 1 0,
  framesep=10pt
]{c}{}{\FL Table's first row\LL}


==> ctable/doc/10b <==
\ctable[
  caption = Frame,
  framerule = 2pt,
  framesep = 5pt,
  framebg = 1 1 0,
  framefg = 1 0 0,
  framesep=10pt
]{c}{}{\FL Table's first row\LL}


==> ctable/doc/12a <==
\ctable{c}{
  \tnote{First note}
  \tnote[b]{Second note}
  \tnote[c]{Third note}
}{\FL Table's\tmark\ first\tmark[b]\ row
      with footnotes\tmark[c]\LL}



==> ctable/doc/12b <==
\ctable[notespar]{c}{
  \tnote[a]{First note.}
  \tnote[b]{Second note.}
  \tnote[c]{Third note, this one is a
            little longer and forces a
            new line at the end.\\}
  \tnote[d]{And here is e very long note:
            \input{thuan}}
}{\FL Table's\tmark\ first\tmark[b]\ row
      with footnotes\tmark[c]\LL}



==> ctable/doc/13a <==
\ctable[
  caption = Caption,
  mincapwidth = 50mm,
]{c}{}{\FL Table's first row\LL}


==> ctable/doc/13b <==
\addtocounter{table}{1} % remove for source
\ctable[
  caption = Caption,
  mincapwidth = 50mm,
  continued
]{c}{}{\FL Table's first row\LL}


==> ctable/doc/13c <==
\addtocounter{table}{1} %remove for source
\ctable[
  caption = Caption,
  mincapwidth = 50mm,
  continued = \textit{(contd)}
]{c}{}{\FL Table's first row\LL}


==> ctable/doc/14a <==
\ctable[
  caption=Doinside,
  doinside = \scriptsize]{l}{
}{\FL
  This table has all rows \NN
  set at script size \LL
}



==> ctable/inst <==
#!/bin/bash
    dtxname=ctable
    dtxtype=package
        ext=sty
     delete=($dtxname.$ext README.tex doc/\*.tex)
 dtxversion=$(grep " v[0-9.]\+[a-z]\{0,1\} $dtxname $dtxtype" $dtxname.dtx |sed 's/.* v\([0-9.]\+[a-z]\{,1\}\) .*/\1/')
executables=(mk texlog_extract zip getopt pdfseparate pdflatex)

    version=1.00
     myname=$(basename $0)

<<'DOC'
= inst - install ctable

= Synopsis
inst [options]	

Without any options, inst installs ctable in the first writable
TEXMFMAIN, TEXMFLOCAL or TEXMFHOME tree.

Options:
-h,--help	print this help and exit
-H,--Help	print full documentation via less and exit
-V,--version	print version and exit


= Description
inst must be run in its own directory (|./inst|) and then does the following:
- generates the documentation for isodoc,
- installs ctable in one of your TeX trees: TEXMFMAIN, TEXMFLOCAL or TEXMFHOME. 
  The first one writable by you will chosen.
- creates a zip file named |ctable-x.yy.zip| for upload to CTAN
- cleans up

= Author and copyright
Author	Wybo Dekker
Email	U{wybo@dekkerdocumenten.nl}{wybo@dekkerdocumenten.nl}
License	Released under the U{www.gnu.org/copyleft/gpl.html}{GNU General Public License}
DOC

    die() { echo -e "$myname: $Err$@$Nor" 1>&2; exit 1; }
   help() { sed -n '/^= Synopsis/,/^= /p' $0|sed '1s/.*/Usage:/;/^= /d'; exit; }
helpall() { sed -n '/^<<.DOC.$/,/^DOC$/p' $0|sed -n '1d;$d;p'|less; exit; }
version() { echo $version; exit; }

Nor='\e[0m'    # reset color	]
Err='\e[31;1m' # light red	]

setdir() { # create installation directory
   for i in MAIN LOCAL HOME; do
      tree=$(kpsewhich --expand-var \$TEXMF$i)
      test -w $tree && break
      tree=
   done
   [[ -n $tree ]] || die "Could not find a writable TeX tree"
   insttex=${tree}/tex/latex/$dtxname
   instsrc=$tree/source/latex/$dtxname
   instdoc=$tree/doc/latex/$dtxname
   mkdir -p $insttex || die could not create $insttex
   mkdir -p $instsrc || die could not create $instsrc
   mkdir -p $instdoc || die could not create $instdoc
}

testexecs() { # test presence of executables
   for i in ${executables[*]}; do
      type $i &> /dev/null || die executable $i not found
   done
}

readme() { # generate the README file
sed -n '/^%<\*readme>/,/^%<\/readme>/p
	/\\changes{v'$dtxversion'}/,/^% }/p' $dtxname.dtx  |
sed    's/^%//;s/\\\\$//
	/ Author:/i\
Version:| '$dtxversion'
	/<.readme>/d
	/^ }/d
	s/ \\changes.*/Changes in version '$dtxversion':/
	s/$\\Rightarrow\$/=>/g
	s/\\textbackslash/\\/g
	s/\\text\(sl\|it\){\([^}]\+\)}/\/\2\//g		# \textsl{...} -> /.../
	s/{\([^}]*\)}/\1/g 				# keep last, removes all {...}
       ' >README
  grep "Changes in version" README >/dev/null || die changes not detected
}

makeall() {
   grep '%<\*install>' $dtxname.dtx >/dev/null && # for self-extracting dtx files
      delete+=($dtxname.ins) ||
      echo y |tex $dtxname.ins >/dev/null

   # install any .ttf files
   mkdir -p ~/.fonts
   find doc -name '*.ttf' -exec cp {} ~/.fonts \;
   fc-cache ~/.fonts

   readme # create the README file

   # compile all examples
   cd doc
   ln -sf ../$dtxname.sty || exit 1 # use the version to be installed
   for i in [0-9][0-9]?; do 
      if [ ! -f $i.pdf -o ! -f s$i.pdf ]; then
         ./doit || exit 1
         break
      fi
   done
   cd ..
  
   mk --noprint --noview $dtxname.dtx && mk -c $dtxname.dtx # make $dtxname.pdf
}

installall() {
   # install and cleanup
   echo installing in $tree

   rm -rf $insttex/* $instsrc/* $instdoc/*
   find doc \( -type l -o -name '*.pdf' \) -delete
   cp -f $dtxname.$ext $insttex
   cp -a $dtxname.{ins,dtx} $instsrc
   cp -a README inst $dtxname.pdf $instdoc
   mktexlsr $tree 2>/dev/null
   for i in ${delete[@]}; do rm -f $i; done 
   cd ..
   zipfile=$dtxname/$dtxname-$dtxversion.zip
   rm -f $zipfile
   zip -rq $zipfile $dtxname/* -x $dtxname/test\*
   cd $dtxname
}

options=$(getopt \
   -n $myname \
   -o hHV \
   -l help,Help,version \
   -- "$@"
) || exit 1
eval set -- "$options"
while [ $# -gt 0 ]; do
   case $1 in
   (-h|--help)	  help;;
   (-H|--Help)	  helpall;;
   (-V|--version) version;;
   (--)		  shift;  break;;
   (*)			  break;;
   esac
done
[[ -z $1 ]] || die No arguments expected

testexecs
setdir
makeall
installall

